Integration and commissioning of the ATLAS Muon spectrometer

The ATLAS experiment at the Large Hadron Collider (LHC) at CERN is currently waiting to record the first collision data in spring 2009. Its muon spectrometer is designed to achieve a momentum resolution of 10% pT(mu) = 1 TeV/c. The spectrometer consists of a system of three superconducting air-core toroid magnets and is instrumented with three layers of Monitored Drift Tube chambers (Cathode Strip Chambers in the extreme forward region) as precision detectors. Resistive Plate Chambers in the barrel and Thin Gap Chambers in the endcap regions provide a fast trigger system. The spectrometer passed important milestones in the last year. The most notable milestone was the installation of the inner layer of endcap muon chambers, which constituted the last big piece of the ATLAS detector to be lowered in the ATLAS cavern. In addition, during the last two years most of the muon detectors were commissioned with cosmic rays while being assembled in the underground experimental cavern. We will report on our experience with the precision and trigger chambers, the optical spectrometer alignment system, the level-1 trigger, and the ATLAS data acquisition system. Results of the global performance of the muon system from data with magnetic field will also be presented.

==> Makefile <==
###############################################################################
#                                                        December 4, 2002
#
# Makefile for a sample CDF Note - Stefan Stonjek  <s.stonjek@physics.ox.ac.uk>
#                                  Martin Hennecke <hennecke@fnal.gov> 
#
###############################################################################

graphics_eps := $(wildcard *.eps)
graphics_pdf := $(patsubst %.eps,%.pdf,$(wildcard *.eps))

ps: atlmuon_abelloni_ichep08.ps
#	gv atlmuon_abelloni_ichep08.ps

pdf: atlmuon_abelloni_ichep08.pdf
#	acroread atlmuon_abelloni_ichep08.pdf

atlmuon_abelloni_ichep08.ps: atlmuon_abelloni_ichep08.tex
	latex atlmuon_abelloni_ichep08.tex && latex atlmuon_abelloni_ichep08.tex && dvips \
	atlmuon_abelloni_ichep08.dvi -o 

atlmuon_abelloni_ichep08.pdf: atlmuon_abelloni_ichep08.tex $(graphics_pdf)
	pdflatex atlmuon_abelloni_ichep08.tex && pdflatex atlmuon_abelloni_ichep08.tex && \
	thumbpdf atlmuon_abelloni_ichep08 && pdflatex atlmuon_abelloni_ichep08.tex

%.pdf: %.eps
	ps2pdf $< $@

.PHONY: clean clear
clear:
	rm -r -f *.aux atlmuon_abelloni_ichep08.dvi atlmuon_abelloni_ichep08.log atlmuon_abelloni_ichep08.out \
	 atlmuon_abelloni_ichep08.toc atlmuon_abelloni_ichep08.lof thumb*.* *~ $(graphics_pdf)    \
        atlmuon_abelloni_ichep08.lot

clean:
	rm -rf *.aux atlmuon_abelloni_ichep08.dvi atlmuon_abelloni_ichep08.log atlmuon_abelloni_ichep08.out    \
	atlmuon_abelloni_ichep08.pdf atlmuon_abelloni_ichep08.ps atlmuon_abelloni_ichep08.toc atlmuon_abelloni_ichep08.lof \
	thumb*.* *~ $(graphics_pdf) atlmuon_abelloni_ichep08.lot


